On statistical inference when fixed points of belief propagation are unstable

Many statistical inference problems correspond to recovering the values of a set of hidden variables from sparse observations on them. For instance, in a planted constraint satisfaction problem such as planted 3-SAT, the clauses are sparse observations from which the hidden assignment is to be recovered. In the problem of community detection in a stochastic block model, the community labels are hidden variables that are to be recovered from the edges of the graph. Inspired by ideas from statistical physics, the presence of a stable fixed point for belief propogation has been widely conjectured to characterize the computational tractability of these problems. For community detection in stochastic block models, many of these predictions have been rigorously confirmed. In this work, we consider a general model of statistical inference problems that includes both community detection in stochastic block models, and all planted constraint satisfaction problems as special cases. We carry out the cavity method calculations from statistical physics to compute the regime of parameters where detection and recovery should be algorithmically tractable. At precisely the predicted tractable regime, we give: (i) a general polynomial-time algorithm for the problem of detection: distinguishing an input with a planted signal from one without; (ii) a general polynomial-time algorithm for the problem of recovery: outputting a vector that correlates with the hidden assignment significantly better than a random guess would.

==> model.tex <==
\section{Setup and notation}

\begin{definition}[Factor type]
	A \emph{factor type} $\phi$ of \emph{arity}-$k$ on domain $\calD$ is a function $\phi:\calD^k\to\R_{\ge 0}$.  Given a factor $\phi$, we use the notation $\arity(\phi)$ to denote $k$, the arity of $\phi$.
\end{definition}


\begin{definition}[Random factor graph]
	A \emph{model} $\Model=(T,\TypeDist,C,\{\ColDist_{\tau}\}_{\tau\in T},\Phi,\Class)$ for random factor graphs is parameterized by a \emph{variable type set} $T$, a distribution $\TypeDist$ over $T$, a \emph{color set} $C$, a distribution $\ColDist_{\tau}$ for every type $\tau\in T$, a \emph{factor type set} $\Phi=\{\phi_1,\dots,\phi_F\}$ where each factor is on domain $C$, and a \emph{factor class function} $\Cl$, which maps each factor type $\phi$ in $\Phi$ to some tuple $(t_1,\dots,t_{\arity(\phi)})$ in $T^{\arity(\phi_i)}$.

	A sample from distribution $\Model^{(n)}$ is a collection $([n],\bE_1,\dots,\bE_F,\btau,\bc)$ drawn in the following way.  $[n]$ is the underlying variable set and each variable $v\in[n]$ is independently assigned a type $\btau(v)\sim\TypeDist$, and a color $\bc(v)\sim\ColDist_{\btau(v)}$.  For each $i\in[F]$ and for each tuple $(v_1,\dots,v_{\arity(\phi_i)})$ of distinct entries in $[n]$ with $\Class(\phi_i) = (\btau(v_1),\dots,\btau(v_{\arity(\phi_i)}))$, we independently sample \emph{type-$i$ factor} $(v_1,\dots,v_{\arity(\phi_i)})$ with probability $\frac{1}{n^{\arity(\phi_i)-1}}\cdot\phi_i(\bc(v_1),\dots,\bc(v_{\arity(\phi_i)}))$.  We define $\bE_i$ as the collection of all sampled type-$i$ factors.
	% A sample from distribution $\Model^{(n)}$ is a collection $([n],\bE_1,\dots,\bE_F,\btau,\bc)$ drawn in the following way.  $[n]$ is the underlying variable set and each variable $v\in[n]$ is independently assigned a type $\btau(v)\sim\TypeDist$, and a color $\bc(v)\sim\ColDist_{\btau(v)}$.  For ease of notation we will use $\bgamma(v)$ to denote the tuple $(\btau(v),\bc(v))$.  For each $i\in[F]$ and for each tuple $(v_1,\dots,v_{\arity(\phi_i)})$ of distinct entries in $[n]$, we independently sample \emph{type-$i$ factor} $(v_1,\dots,v_{\arity(\phi_i)})$ with probability $\frac{1}{n^{\arity(\phi_i)-1}}\cdot\phi_i(\bgamma(v_1),\dots,\bgamma(v_{\arity(\phi_i)}))$.  We define $\bE_i$ as the collection of all sampled type-$i$ factors.

	We treat $\bG$ as a bipartite graph where the left vertex set is given by the variables $[n]$ and the right vertex set is given by the collection of all $(i,(v_1,\dots,v_{\arity(\phi_i)}))$ for factor $(v_1,\dots,v_{\arity(\phi_i)})\in \bE_i$.  For $e = (i,(v_1,\dots,v_{\arity(\phi_i)}))$ we define $\index_e(v_s)$ as $s$ and define $e[s]$ as $v_s$.  When $e$ is clear from context, we shall drop the $e$ and simply use $\index(v_s)$ to denote $\index_e(v_s)$.  Given a factor $e$, we use $\FacType(e)$ to denote its type.
\end{definition}

\begin{remark}
	For a model with $F$ factors $\phi_1,\dots,\phi_F$, we will abuse notation and use $\arity(i)$ to denote $\arity(\phi_i)$, and $\Cl(i)$ to denote $\Cl(\phi_i)$.
\end{remark}

\begin{definition}[Null and Planted distributions]	\label{def:null-planted}
	Let $\Model_{\scn}$ and $\Model_{\scp}$ be two models such that:
	\begin{enumerate}
		\item the variable type sets of the models are both equal to $T$,
		\item the number of factor types of the models are both equal to $F$,
		\item for every $i\in[F]$ the arity and factor class of the type-$i$ factors in the models $\Model_{\scn}$ and $\Model_{\scp}$ are equal,
		\item and the color set $C_{\scn}$ of $\Model_{\scn}$ is the singleton set $\{1\}$.
	\end{enumerate}
	Now, let $\bG$ be a sample from the \emph{null distribution} $\Null$ defined in the following way:
	\begin{enumerate}
		\item Let $([n],\bE_1,\dots,\bE_F,\btau,\bc)$ be a sample from $\Model_{\scn}^{(n)}$.
		\item Let $\bG \coloneqq ([n],\bE_1,\dots,\bE_F,\btau)$.
	\end{enumerate}
	Likewise, we define a sample $\bG$ from the \emph{planted distribution} $\Planted$ in the following analogous way:
	\begin{enumerate}
		\item Let $([n],\bE_1,\dots,\bE_F,\btau,\bc)$ be a sample from $\Model_{\scp}^{(n)}$.
		\item Let $\bG \coloneqq ([n],\bE_1,\dots,\bE_F,\btau)$.
	\end{enumerate}
\end{definition}

\begin{question}	\label{que:distinguisher}
	Let $\Model_{\scn}$ and $\Model_{\scp}$ be two models satisfying the conditions in \pref{def:null-planted}.  Let $\Null$ and $\Planted$ be the corresponding null and planted distributions on $n$ variables.  Given $\bG$ sampled from either $\Null$ or $\Planted$ is there a $\poly(n)$-time algorithm that correctly outputs ``null'' if $\bG\sim\Null$ and ``planted'' if $\bG\sim\Planted$ with probability $1-o_n(1)$.
\end{question}



==> weak-recovery.tex <==
\section{A weak recovery algorithm }

We are interested in the problem of reconstructing a hidden assignment $\bc$ from an observation $([n],\bE_1,\dots,\bE_F,\btau)$ from the planted model $\bP$. Here the hidden assignment and the observation are jointly sampled as $\bG =([n],\bE_1,\dots,\bE_F,\btau)\sim\Model^{[n]}_{\scp}$.

Recall that we denote the observation's centered adjacency matrix $\CentAdj_{\bG}\in\R^{\abs{C}n\times\abs{C}n}$. The matrix consists of blocks $\CentAdj_{\bG}[u,v]\in\R^{\abs{C}\times\abs{C}}$ $(u,v\in[n])$ which are defined as 

\[\CentAdj_{\bG}^{(s)}[u,v] = \sum_{e \mid e\ni u,v} \bTrans_{\FacType_e,\btau(u)\mid\btau(v)} \left(\mathbf{1}[e\in\bG] - \Pr_{\bG'}[e\in\bG']\right) .\] \siqi{Is the use of $\FacType_e$ correct?}

Let $E_{\btau,\bc} = \E_{\bG}[\CentAdj_{\bG}| \btau,\bc]$.  Let $\CentAdj_{\bG,c} = \CentAdj_{\bG} - E_{\btau,c}$ and let $\CentAdj_{\bG,\bc}^{(\ell)}$ denote its $\ell$-th nonbacktracking power.  Note that for any distinct $u,v\in[n]$ of a given type $\tau$ and color $c$, the $(u,v)$ block of $E_{\btau,\bc}$ contains matrix $E_{\btau,c}(\tau,c)$ depending only on $\tau$ and $c$.  Thus, we define $F_{\btau,\bc}$ be the $|C|\cdot n\times |C|\cdot n$ matrix obtained by taking $E_{\btau,\bc}$ and additionally placing matrix $E_{\btau,\bc}(\btau(v),\bc(v))$ in the $(v,v)$-block for all $v\in[n]$.

Also recall that the vector $\statvec_{\bG}\in\R^{\abs{C}n}$ is the concatenation of $n$ indicator vectors $\statvec_v\in\R^{\abs{C}}$ for $(v\in[n])$ with $\ColDist_{\tau(\bv)}(c)$ subtracted from every coordinate $(v,c)$. % Each $\statvec_v$ is nonzero at the entry indicating its true assignment $\bc(v)$. 

Given a vector in $\R^{|C|\cdot n}$ we treat it as a block vector comprising of $n$ blocks of dimension $|C|$ each where each block corresponds to a vertex in $[n]$.  Now, we define a $|C|\cdot n\times|C|\cdot n$-dimensional positive diagonal matrix $\innerp_{\btau}$ where the $(v,v)$ block is equal to:
\[
	\innerp_{\btau,(v,v)}[c,c] \coloneqq \ColDist_{\btau(v)}(c)
\]
We will use the following inner product on $\R^{|C|\cdot n}$:
\[
	\langle x, y\rangle \coloneqq x^{\top}\innerp_{\btau}^{\dagger}y.
\]
where $\innerp_{\btau}^{\dagger}$ denotes the pseudoinverse of $\innerp_{\btau}$.\footnote{An astute reader will observe that when some $\ColDist_{\btau}(c)$ is $0$, the below does not satisfy the positive definite property required of an inner product.  Nevertheless, it is still a valid inner product on the subspace spanned by coordinates $(v,c)$ where $\ColDist_{\btau(v)}(c)$ is nonzero, and this subspace contains all the vectors we work with and is in the kernel of all the matrices we work with.}
\begin{lemma}	\label{lem:self-adj}
	The matrices $\Adj_{\bG}$, $\CentAdj_{\bG}$ and $F_{\btau,\bc}$ are self adjoint under $\langle \cdot, \cdot\rangle$.
\end{lemma}
\sid{somewhere gotta prove that all these matrices we care about are self-adjoint under the above inner product.  This can be proved using some stuff in calculus.tex.  \pref{app:calculus}}

We now describe our algorithm for weak recovery.
\begin{itemize}
	\item Let $s \coloneqq \frac{\log n}{(\log\log n)^2}$ and $\kappa = \frac{\lambda_L^s}{\log\log n}$.
	\item Compute eigenvectors of $\CentAdj_{\bG}$ and let $\rvec_1,\dots,\rvec_m$ be an orthogonal basis of eigenvectors corresponding to eigenvalues of magnitude greater than $\kappa$.
	\item Let $\bw$ be a uniformly random vector on the $m$-dimensional unit sphere.
	\item Output $\rvec \coloneqq \bw[1]\rvec_1 + \dots + \bw[m]\rvec_m$.
\end{itemize}



% \begin{definition}
% $\CentAdj_{\btau,\bc} = \E_{\bG}[ \CentAdj_{\bG} \mid \btau,\bc]$
% \end{definition}

We prove the following weak recovery theorem.
\begin{theorem}\label{thm:weak-recovery}
	There exists an absolute constant $\alpha_{\ref{thm:weak-recovery}}$ such that the output $\rvec$ of the above algorithm satisfies:
	\begin{align*}
		\|\rvec\|^2 &= 1 \\
		\E\langle \rvec, \statvec_{\bG} \rangle^2 &\ge \alpha_{\ref{thm:weak-recovery}}\cdot\|\statvec_{\bG}\|^2
	\end{align*}
\end{theorem}

% \begin{theorem}\label{thm:weak-recovery} 
% Let $\calA$ be the algorithm that on input $\CentAdj_{\bG}$ computes its eigenvectors $\rvec_1,\dots,\rvec_m$ whose eigenvalues $\gg n^{\Theta(1/\log\log{n})}$, and outputs $\rvec := \sum_{i=1}^m \rvec_i / m$. The output $\rvec$ satisfies that \siqi{I set $s = \Theta(\log{n}/\log{\log{n}})$. Not sure if we can really get this. The approach I wrote down has gaps.}
% \[ \Pr_{\bG\sim\Model^{[n]}_{\scp}}[ \langle \rvec,\statvec_{\bG} \rangle \geq \epsilon n] \geq 1 - o_n(1) .\]
% \end{theorem}

We shall prove \pref{thm:weak-recovery} using the following lemmas. Proofs of the lemmas are in the appendix.\sid{insert references to the appendix section(s?) when done.}

\begin{lemma}\label{lem:m-constant}
	Let $m$ be the number of eigenvalues of $\CentAdj_{\bG}$ that exceed $\kappa$ in magnitude.  With probability $1-o(1)$, $m$ is bounded by an absolute constant.
\end{lemma}

\begin{lemma}\label{lem:loc-stat}
	There exists an absolute constant $\alpha_{\ref{lem:loc-stat}}$ such that with probability $1-o(1)$: $\langle \statvec_{\bG}, \CentAdj_{\bG}^{(s)}\statvec_{\bG}\rangle\ge\alpha_{\ref{lem:loc-stat}}\lambda_L^s\|c\|^2$.
\end{lemma}

\begin{lemma}\label{lem:bdd-spec-norm}
	There exists an absolute $\alpha_{\ref{lem:bdd-spec-norm}}$ With probability $1-o(1)$: $|\lambda|_{\max}(\CentAdj_{\bG}^{(s)}) \le \alpha_{\ref{lem:bdd-spec-norm}}\lambda_L^s$.
\end{lemma}

Now, we prove \pref{thm:weak-recovery} assuming the above three lemmas.
\begin{proof}[Proof of \pref{thm:weak-recovery}]
	Since $\CentAdj_{\bG}^{(s)}$ is self-adjoint by \pref{lem:self-adj}, it has an orthogonal basis of eigenvectors $u_1,\dots,u_{|C|\cdot n}$ with eigenvalues $\lambda_1,\dots,\lambda_{|C|\cdot n}$, and hence $\|\rvec\|^2 = \|\bw\|^2 = 1$.  To prove the second part, first write $\statvec_{\bG}$ in the basis of eigenvectors of $\CentAdj_{\bG}$ as follows:
	\[
		\statvec_{\bG} = \sum_{i=1}^{|C|\cdot n} \mu_i \rvec_i.
	\]
	From \pref{lem:loc-stat}:
	\begin{align*}
		\alpha_{\ref{lem:loc-stat}}\lambda_L^s\|\statvec_{\bG}\|^2 &\le \langle \statvec_{\bG}, \CentAdj_{\bG}^{(s)}\statvec_{\bG}\rangle\\
		&= \left\langle \sum_{i\ge1} \mu_i \rvec_i, \sum_{i\ge 1} \mu_i\lambda_i\rvec_i \right\rangle\\
		&= \sum_{i\ge 1} \lambda_i \mu_i^2
		\intertext{By \pref{lem:bdd-spec-norm}}
		&\le \alpha_{\ref{lem:bdd-spec-norm}} \sum_{i=1}^m \mu_i^2 + \kappa \|\statvec_{\bG}\|^2.
	\end{align*}
	This inequality along with the choice of $\kappa$ implies:
	\[
		\sum_{i=1}^m \mu_i^2 \ge \frac{\alpha_{\ref{lem:loc-stat}}}{\alpha_{\ref{lem:bdd-spec-norm}}} - O\left(\frac{1}{\log\log n}\right) \ge \zeta
	\]
	for an absolute constant $\zeta$.  Now:
	\begin{align*}
		\E\langle \bw, \statvec_{\bG}\rangle^2 = \E\left[\left(\sum_{i=1}^m \bw[i]\mu_i\right)^2\right] = \frac{\sum_{i=1}^m\mu_i^2}{m},
	\end{align*}
	which is equal to a constant which we call $\alpha_{\ref{thm:weak-recovery}}$.
\end{proof}

\begin{lemma}\label{lem:orthogonal-to-centered-color}
Set $s:= \Theta(\log{n}/\log{\log{n}})$.

For any $x\in\R^{\abs{C}n}$ such that $\norm{\CentAdj_{\bG}^{(\ell)}\CentAdj_{\btau,\bc} x}_2 \leq \epsilon(n)\norm{x}_2$ for all $\ell\in[s]$, $x^T\CentAdj_{\bG}^{(s)}x = o(n^{\Theta(1/\log\log{n})}) $.

Or alternatively: For any $x^T\CentAdj_{\bG}^{(s)}x = \Omega(n^{\Theta(1/\log\log{n})})$, $\norm{\CentAdj_{\btau,\bc} x}_2 > \epsilon(n)\norm{x}_2$. \siqi{Fill in $\epsilon(n)$, should be superconstant.}
\end{lemma} 

\begin{lemma}
$\CentAdj_{\btau,\bc}$ has no eigenvalues $\leq \epsilon(n)- O(1)$.
\end{lemma}

\begin{proof}
Let $\rvec_1,\dots,\rvec_m$ denote the eigenvectors of $\CentAdj_{\bG}$ whose eigenvalues $\gg n^{\Theta(1/\log\log{n})}$.

We first show that $m$ must be a constant and that all $\rvec_i$ and also the true assignment $\statvec_{\bG}$ are heavily correlated to $\CentAdj_{\btau,\bc}$. 

For any vector $v$ 
\[v^T\CentAdj_{\bG}^{(s)}v = v^T\left(\CentAdj_{\bG}^{(s)} - \CentAdj_{\btau,\bc}^{(s)}\right)v + v^T \CentAdj_{\btau,\bc}^{(s)} v .\]

With probability $1 - o_n(1)$ over $\bG$, the first term $v^T\left(\CentAdj_{\bG}^{(s)} - \CentAdj_{\btau,\bc}^{(s)}\right)v$ is bounded by $\norm{v}^2_2$, since by \pref{thm:main-spectral-bound} \siqi{more explanation here} $\norm{\CentAdj_{\bG}^{(s)} - \CentAdj_{\btau,\bc}^{(s)}}_{op} < 1$. Thus 
\[v^T \CentAdj_{\btau,\bc}^{(s)} v > v^T\CentAdj_{\bG}^{(s)}v - \norm{v}^2_2.\]

Thus by definition of $\rvec_i$ and by \pref{lem:local-statistics-expectation}, with probability $1 - o_n(1)$ over $\bG$
\[\rvec_i^T \CentAdj_{\btau,\bc}^{(s)} \rvec_i = \Omega\left(n^{\Theta(1/\log\log{n})}\right), \quad \statvec_{\bG}^T \CentAdj_{\btau,\bc}^{(s)} \statvec_{\bG} = \Omega\left(n^{\Theta(1/\log\log{n})} n\right) .\] 

Then we can apply \pref{lem:orthogonal-to-centered-color} and dedue that $\norm{\CentAdj_{\btau,\bc}\rvec_i}_2 > \epsilon(n)$ and $\norm{\CentAdj_{\btau,\bc}\statvec_{\bG}}_2 > \epsilon(n) n $. 

Although $\CentAdj_{\btau,\bc}$ has high rank, it is close in Forbenius norm to a constant rank matrix $\CentAdj_{\btau,\bc}'$. Thus after the rank reduction $\norm{\CentAdj_{\btau,\bc}'\rvec_i}_2 > \epsilon(n) - O(1)$ and $\norm{\CentAdj_{\btau,\bc}'\statvec_{\bG}}_2 > (\epsilon(n) - O(1)) n$. Since $\CentAdj_{\btau,\bc}'$ has constant rank, and all the vectors $\rvec_1,\dots,\rvec_m$ are orthogonal vectors in the column space of $\CentAdj_{\btau,\bc}'$, we deduce that $m = \Theta(1)$. Therefore the algorithm $\calA$ is efficient.

[This is not true for SBM even, I think....]Furthermore, $\rvec_1,\dots,\rvec_m$ spans the eigen subspace of $\CentAdj_{\btau,\bc}$ of eigenvalues $\gg o(\epsilon(n))$. This is because by \pref{lem:orthogonal-to-centered-color} any $x$ in this eigen subspace (i.e. $\norm{\CentAdj_{\btau,\bc} x}_2 \geq \epsilon(n)\norm{x}_2$) 

Then it immediately follows that $\left\langle \rvec, \statvec_{\bG} \right\rangle = \left\langle\frac{1}{m} \sum_{i=1}^m \rvec_i, \statvec_{\bG} \right\rangle \geq \frac{1}{m}\norm{\CentAdj_{\btau,\bc}\statvec_{\bG}}_2 - o(\epsilon(n))n = \Theta(\epsilon(n))n$. 
\end{proof}


XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX\sid{Just writing separately for now --- there might be overlapping notation -- will unify all of that soon.}
\subsection{Weak Recovery Prime}
Let $E_{\btau,\bc} = \E_{\bG}[\CentAdj_{\bG}| \btau,\bc]$.  Let $\CentAdj_{\bG,c} = \CentAdj_{\bG} - E_{\btau,c}$ and let $\CentAdj_{\bG,\bc}^{(\ell)}$ denote its $\ell$-th nonbacktracking power.  Note that for any distinct $u,v\in[n]$ of a given type $\tau$ and color $c$, the $(u,v)$ block of $E_{\btau,\bc}$ contains matrix $E_{\btau,c}(\tau,c)$ depending only on $\tau$ and $c$.  Thus, we define $F_{\btau,\bc}$ be the $|C|\cdot n\times |C|\cdot n$ matrix obtained by taking $E_{\btau,\bc}$ and additionally placing matrix $E_{\btau,\bc}(\btau(v),\bc(v))$ in the $(v,v)$-block for all $v\in[n]$.
\begin{definition}
	We define the complete factor graph $\CompG_{\Model^{[n]}}=([n],E_1,\dots,E_F)$ as the instance where $E_i$ denotes the collection of all potential type-$i$ factors that could appear in $\bG\sim\Model^{[n]}$.
\end{definition}
Given a vector in $\R^{|C|\cdot n}$ we treat it as a block vector comprising of $n$ blocks of dimension $|C|$ each where each block corresponds to a vertex in $[n]$.  Now, we define a $|C|\cdot n\times|C|\cdot n$-dimensional positive diagonal matrix $\innerp_{\btau}$ where the $(v,v)$ block is equal to:
\[
	\innerp_{\btau,(v,v)}[c,c] \coloneqq \ColDist_{\btau(v)}(c)
\]
We will use the following inner product on $\R^{|C|\cdot n}$:
\[
	\langle x, y\rangle \coloneqq x^{\top}\innerp_{\btau}^{\dagger}y.
\]
where $\innerp_{\btau}^{\dagger}$ denotes the pseudoinverse of $\innerp_{\btau}$.\footnote{An astute reader will observe that when some $\ColDist_{\btau}(c)$ is $0$, the below does not satisfy the positive definite property required of an inner product.  Nevertheless, it is still a valid inner product on the subspace spanned by coordinates $(v,c)$ where $\ColDist_{\btau(v)}(c)$ is nonzero, and this subspace contains all the vectors we work with and is in the kernel of all the matrices we work with.}
\begin{lemma}
	The matrices $\Adj_{\bG}$, $\CentAdj_{\bG}$ and $F_{\btau,\bc}$ are self adjoint under $\langle \cdot, \cdot\rangle$.
\end{lemma}
\sid{somewhere gotta prove that all these matrices we care about are self-adjoint under the above inner product.  This can be proved using some stuff in calculus.tex.  \pref{app:calculus}}
\begin{definition}
	For a given $\tau:[n]\to T$ and $c:[n]\to C$ we say a vector $v$ in $\R^{|C|\cdot n}$ is \emph{$(\tau,c)$-symmetric} if there exist vectors $\{u_{\tau,c}\}_{(\tau,c)\in T\times C}$ such that for any vertex $i$, the $i$-th block of $v$ is equal to $u_{\tau(i),c(i)}$ and for every $(\tau,c)\in T\times C$ we have $\langle u_{\tau,c}, \ColDist_{\tau} \rangle = 0$.  Henceforth, we will use $V_{\tau,c}$ to denote the set of all vectors that are $(\tau,c)$-symmetric.
\end{definition}
\begin{observation}
	$V_{\tau,c}$ is a vector space of dimension $|T|\cdot(|C|-1)$.
\end{observation}
\begin{lemma}
	The column space of $F_{\btau,\bc}$ is contained in $V_{\btau,\bc}$.
\end{lemma}
\sid{insert proof}

Here is an outline of how we prove that the number of ``outlier'' eigenvectors of $\Adj_{\bG}$, i.e., the number of eigenvectors with eigenvalue larger than threshold $\kappa$, is at most $|T|\cdot(|C|-1)$.
\begin{enumerate}
	\item Our guess for a subspace that heavily correlates with the outlier eigenvectors is $W_{\btau,\bc}\coloneqq \{\Adj_{\bG}^{(s)}v:v\in V_{\btau,\bc}\}$.
	\item We will prove that for any $x$ orthogonal to $W_{\btau,\bc}$, the quadratic form $\langle x, \Adj_{\bG}^{(s)} x\rangle \le \eps(n)\kappa$ where $\eps(n)$ is some decaying function in $n$.  The variational characterization of eigenvalues given by the Courant-Fischer theorem then tells us that there are at most $|T|\cdot(|C|-1)$ eigenvalues exceeding $\eps(n)\kappa$, and hence there are definitely only at most $|T|\cdot(|C|-1)$ eigenvalues exceeding $\kappa$ in magnitude.  % We then illustrate that this implies for any eigenvector $v$ with eigenvalue at least $\kappa$, most of $v$ lives in $W_{\btau,\bc}$ --- concretely, $\langle v, \Pi_{\btau,\bc}v\rangle \ge (1-\eps(n))\langle v,v\rangle$ where $\Pi_{\btau,\bc}$ is the orthogonal projection onto $W_{\btau,\bc}$.
	\item 
\end{enumerate}




